Multi-Objective Congestion Control

Decades of research on Internet congestion control (CC) has produced a plethora of algorithms that optimize for different performance objectives. Applications face the challenge of choosing the most suitable algorithm based on their needs, and it takes tremendous efforts and expertise to customize CC algorithms when new demands emerge. In this paper, we explore a basic question: can we design a single CC algorithm to satisfy different objectives? We propose MOCC, the first multi-objective congestion control algorithm that attempts to address this challenge. The core of MOCC is a novel multi-objective reinforcement learning framework for CC that can automatically learn the correlations between different application requirements and the corresponding optimal control policies. Under this framework, MOCC further applies transfer learning to transfer the knowledge from past experience to new applications, quickly adapting itself to a new objective even if it is unforeseen. We provide both user-space and kernel-space implementation of MOCC. Real-world experiments and extensive simulations show that MOCC well supports multi-objective, competing or outperforming the best existing CC algorithms on individual objectives, and quickly adapting to new applications (e.g., 14.2x faster than prior work) without compromising old ones.

==> sections/1intro.tex <==
\section{Introduction}\label{sec:intro}%\vspace{-1mm}
\vspace{-0.15in}

\iffalse
\begin{table*}[ht]
\vspace{-5mm}
\footnotesize
\begin{tabular}{m{6cm}<{\centering}|m{4cm}<{\centering}|m{3cm}<{\centering}|m{3cm}<{\centering} }
\hline
\multirow{2}{4em}{\textbf{Applications}} & \multicolumn{3}{c}{\textbf{Performance requirements/demands}}\\
\cline{2-4}
& Throughput(bps) & Latency(ms), Jitter(ms) & Packet Loss Rate\\
\hline
\hline
Web Browsing (Normal/Enhanced)~\cite{qos}         & $<$24K(30.5K)   &$<$400 , N/A        & N/A \\
Email/FTP/Telnet~\cite{qos}                       & $<$10K/5K/1K    &Low/Med/High , N/A  & N/A \\
Internet Relay Chat~\cite{qos}                    & $<$1K           &$<$200 , N/A        & $<$0.1\% \\
Audio/Video Broadcasting~\cite{kenyon1992audiovisual}~\cite{silveira1999multimedia}              & 80K(40M)     &$<$100 , $<$100     & $<$1\%(0.1\%) \\
Audio/Video Conferencing~\cite{fluckiger1995understanding}                & 17K(80K)     &$<$150 , $<$400     & $<$1\%(0.1\%) \\
Multimedia on Web~\cite{silveira1999multimedia}                       & $>$28.8-500K    &$<$150 , $<$150     & $<$0.01\% \\
Telemetry~\cite{qos}                               & 2K-52M       &$<$250 , $<$100     & N/A \\
Autonomous Driving~\cite{qos1}                       & 10M          &$<$15  , $<$400     & Zero \\
Device Remote Controlling~\cite{qos1}               & 5M           &$<$100 , $<$100     & Zero \\
Personal Cloud~\cite{qos1}                          & 10M          &$<$1000, N/A        & N/A \\
Voice Over IP~\cite{szuprowicz1995multimedia}                           & 17K          &$<$100 , $<$ 400    & $<$1\% \\
Virtual Reality (Entry/Advanced/Extreme)~\cite{qos1}& $>$100M/400M/1G &$<$100 , $<$30/20/1 & $<$1\% \\
Augmented Reality~\cite{qos1}                       & $>$100M     &$<$10      &$<$1\% \\
Tactile Internet~\cite{qos1}                        & $>$1G           &$<$10  , N/A        & Zero \\
\hline
\end{tabular}
\caption{Examples of some Internet applications and their requirements on underlying network performance}\label{table:app}
\vspace{-2em}
\end{table*}
\fi

Today's Internet carries a variety of classic and emerging applications with diverse performance requirements characterized by metrics such as throughput, latency, and loss rate ($\S$\ref{subsec:appreq}). Some require high-throughput, while others desire low latency with low packet loss. To support these applications, an ideal underlying congestion control (CC) algorithm should be: 1) {\em application-aware} to meet each application-specific demand, 2) {\em multi-objective} to support multiple application requirements simultaneously, and 3) {\em quick-adaptive} to accommodate new arrival applications. %with new requirements.

Despite decades of efforts, there is still a significant gap between the network
stack and the upper-layer applications.
To the best of our knowledge, almost all existing congestion control algorithms, from traditional hand-crafted heuristics (e.g.,~\cite{vegas, cubic, newreno, compound, bbr, copa, fast}) to recent learning-based schemes (e.g.,~\cite{remy, allegro, vivace,aurora}), do not meet the above goals. On one hand, most traditional heuristic algorithms have no explicit application-aware utility function and hardwiredly map packet-level events to pre-defined control rules based on human experiences, thus hard to achieve optimal application-specific performance. State-of-the-art learning algorithms (e.g., Aurora~\cite{aurora}), on the other hand, are application-aware since they explicitly specify application-specific performance objective in utility/reward function and maximize it through machine learning from network environments. However, the key problem is that they can only optimize for a single objective at a time, due to the model's inability to recognize different applications. As a result, supporting multiple different applications requires multiple models, and furthermore, adapting to a new application entails re-training a model from scratch which takes long time (see Figure~\ref{fig:moti}c), making it neither multi-objective nor quick-adaptive (details in $\S$\ref{subsec:problem}).

This paper takes the initiative in addressing the challenge by proposing \sys, a multi-objective congestion control framework that aims to achieve all the above three goals simultaneously ($\S$\ref{sec:MORL}). We are inspired by prior work to build \sys on top of Reinforcement Learning (RL) which has already been shown to achieve optimal single-objective performance~\cite{aurora}. However, to enable multi-objective, we make key improvement upon prior single-objective RL by explicitly incorporating the application requirements into both state inputs and dynamic reward functions, and designing a new policy neural network with a preference sub-network that correlates these different application requirements with optimal rate control policies correspondingly ($\S$\ref{subsec:architecture}). In this way, \sys effectively establishes {\em a single correlation model} that supports multiple applications simultaneously, even with conflicting requirements.

We further leverage transfer learning techniques~\cite{meta,neighbour} to achieve quick-adaptation for new arrival applications. For this purpose, we first pre-train \sys on a well-distributed set of landmark objectives to learn the base correlations between application requirements and optimal policies ($\S$\ref{subsec:offline}). Then, for a new application, \sys is capable of providing a moderate policy of sending rate even it is unseen before. Meanwhile, transferring from such base correlation model, \sys can quickly converge to the optimal model for the new application with just a few RL iterations, much faster than learning from scratch. Furthermore, to avoid forgetting the already learned policies for old applications, we modify the loss function of the online learning by optimizing for both the new arrival and sampled history applications, so that \sys can recall the learned policies for old applications. As a result, our \sys framework is able to learn and apply optimal policies to new applications on-the-fly, without compromising old ones ($\S$\ref{subsec:online}).

We provide two implementations of \sys, a user-space implementation
with UDT~\cite{udt} and a kernel-space implementation with CCP~\cite{ccp}.
The design components are fully implemented based on OpenAI
Gym~\cite{openai}\footnote{OpenAI Gym is a widely adopted toolkit to implement
RL.} and Aurora~\cite{aurora}. We adopt parallel training to further accelerate
the training of \mocc. For better portability, we encapsulate all \mocc's
functions into one library that is plug-and-play and readily deployable with any
networking datapaths.

%\TODO{to polish, Kai will do} This paper introduces a multi-objective congestion control (MOCC) framework that aims to achieve all the above three goals simultaneously. We are inspired by prior work~\cite{aurora} to build MOCC on top of Reinforcement Learning (RL) which has already been shown to achieve optimal single objective performance. However, to support multi-objective, we improve up on prior single objective RL by explicitly incorporating the application preferences into both the state input and the dynamic reward function, and designing a new policy neural network that maps both the observed network states and the application preferences to the sending rate. In this way, MOCC can easily express multiple objectives and support multiple applications simultaneously.

%We further leverage transfer learning technology to achieve quick-adaption for new arrival applications. For this purpose, we pre-train our MOCC model with a wide range of weight combinations to learn the correlations between the application objectives and the optimal policies. Then, for a new objective, our model is capable of generating a moderate policy of sending rate even it is unseen before. Meanwhile, transferring from such a moderate policy, MOCC can quickly converge to the optimal policy for the new application, much faster than learning from scratch. In addition, to avoid forgetting the already learned policies for existing applications, we modify the loss function of the online learning by optimizing on both the new arrival and sampled history applications, so that MOCC can recall the learned policies for previous applications. As a result, our MOCC framework is able to learn, memorize and enforce policies on-the-fly as application changes.

%We implement MOCC \TODO{finish this, Junxue}.
%The implementation of \mocc contains three major parts: 1) offline training simulator; 2) \mocc online adaptation library and 3) application integration layer. The training simulator is based on OpenAI Gym~\cite{} and we adopt parallel training to further accelerate the training of \mocc. Furthermore, the well-encapsulated library makes \mocc a plug-and-play solution, which is easy to be integrated with various datapath implementations. Finally, we integrate \mocc with UDT~\cite{} and CCP~\cite{} in our application integration shim layer, to provide both user-space and kernel-space \mocc implementations.
%We compare \sys with a series of representative Internet CC algorithms using extensive simulations and experiments with real Internet applications. Our main highlights include:

We finally evaluate \sys using extensive simulations, real Internet experiments and deep-dive analysis ($\S$\ref{sec:eva}). Our main findings include:
\begin{icompact}
\item \textbf{Multi-objective:} We compare \mocc against a variety of heuristic and learning-based CC algorithms in terms of meeting different application requirements ($\S$\ref{subsec:AA}). Our results show that \mocc well enables different applications and is able to rival or outperform the best existing schemes under different scenarios (Figure~\ref{fig:multi1} and~\ref{fig:cdf}).

\item \textbf{Quick-adaptation:} We compare \mocc with the state-of-the-art RL CC algorithm Aurora~\cite{aurora} in terms of adapting to new applications ($\S$\ref{subsec:QA}). We find that, for a new application, \mocc can start from a good policy and quickly converge to the optimal policy in 4.8 minutes, $14.2\times$ faster than Aurora (Figure~\ref{fig:quick}a). We also observe that \mocc does not compromise old applications when adapting to the new one, whereas Aurora does, significantly (Figure~\ref{fig:quick}b).

\item \textbf{Real Internet applications:} We showcase the performance of \mocc with 3 real Internet applications: video streaming, real-time communications (RTC), and bulk data transfer ($\S$\ref{subsec:realapp}). Our results demonstrate that \mocc is able to provide high bitrate/throughput for video streaming (Figure~\ref{fig:vs}) and bulk data transfer (Figure~\ref{fig:bdt}), while delivering the lowest inter-packet latency for RTC (Figure~\ref{fig:rtc}).

\item \textbf{Deep-dive:} Finally, we deep-dive into \mocc from a series of other aspects ($\S$\ref{subsec:DD}) such as the choices of hyperparameters (Figure~\ref{fig:finegrain}), learning algorithm (Figure~\ref{fig:model}), training speedup techniques (Figure~\ref{fig:speedup}), etc., to validate its design decisions. Finally, we inspect \mocc's fairness (Figure~\ref{fig:fair}) and TCP-friendliness (Figure~\ref{fig:friend}).
\end{icompact}

%This work does not raise any ethical issues.


\begin{figure*}[ht]
\centering
\subfigure[Support for throughput-sensitive application] {
    \includegraphics[width=0.32\textwidth]{image/tput-new.pdf}
  }
\subfigure[Support for latency-sensitive application]{
    \includegraphics[width=0.32\textwidth]{image/delay-1.pdf}
  }
\subfigure[Time cost of re-training for new application]{
    \includegraphics[width=0.32\textwidth]{image/reward-1.pdf}
  }
\vspace{-3mm}
\caption{Showcases of different CC algorithms in supporting for throughput-sensitive application (a) and latency-sensitive application (b). TCP CUBIC is good for throughput but bad for latency. Vegas is good for latency but bad for throughput. Aurora performs the best in both throughput and latency, but with two different models, and re-training the model takes long time (c).}
\label{fig:moti}
\vspace{-0.15in}
\end{figure*}


\vspace{-0.1in}



%MOCC formalizes congestion control task as a multi-objective reinforcement learning problem. Different from single-objective RL model applied by [PCCRL], it can learn how to choose sending rate over multiple metrics with arbitraly given preferences, such as latency, throughput and packet loss. To make our model aware of the current objective, we incorparate the preferences of metrics into the input features as weight vector. A policy neural network is designed to map both the observations and the preferences to the sending rate decision for the next time interval. In this way, our algorithm can explicitly express various application requirements simultaneously by adjusting the preferences input. Furthermore, to enable training and evaluation on multiple objectives, we parameterize the reward/feedback of the network environment with the preference weights to respect the requirements. During training, the model makes rate control decisions for applications with different requirements, obtains the corresponding rewards, and learns to optimize its policy for each objective through history experience.

%To achieve quick-adaptation for new coming applications, we adopt a online learning scheme for our model. In the offline phase, we pre-train our model with a wide range of preference weight combinations to learn the correlation between objective preferences and the optimal policy. So for emerging application with new requirement, our preference network can generate a moderate policy to decide the sending rate considering new metric preferences. In the online phase, our algorithm continues to learn with new experiences during deployment. Transferring from the moderate policy, our model can converge to the optimal policy for new application requirements more quickly than learning from scratch. In the meanwhile, to avoid forgetting the already learned policies, we modify the loss function for online learning by optimizing on both the current and sampled history application requirements, so that our model can recall the learned policies for previous applications. As a result, the MOCC framework is able to learn, memorize and enforce policies on-the-fly as application changes.


%\pho{rewrite here }
%
%We pre-trained our \mocc in a network simulator provided by Aurora~\cite{x}. We evaluate \sys using a full system implementation. Our implementation includes two parts. \emph{First part},  we integrates \mocc into the comprehensive emulator Pantheon~\cite{x}. \emph{Furthermore}, we deploys \mocc into CCP~\cite{x} and thus \mocc can be used in datapath Linux Kernel TCP. We also implement two real application, video streaming based on Pensieve~\cite{x}, and WebRTC based on Salsify~\cite{x}. Thus we could test the \mocc both under emulated realistic network conditions (Pantheon) and in the real-world internet and in application scenarios.
%
%\yq{7.Evaluation}
%
%We compare \mocc to the state-of-the-art congestion control algorithms using a broad set of network conditions also for a broad set of network applications. \emph{Firstly}, in a mixed applications scenario, our \mocc significantly outperforms the best existing scheme in the generalization ability for \wait{xx} percentage, which shows \mocc's ability for application awareness far beyond the existing learning-based method and heuristic handcrafted methods. \emph{Furthermore}, we build experiments to show that \mocc has the ability of quick adapting to unseen applications' demands compared with other learning-based cc (PCC-Vivace, PCC-Allegro, PCC-Aurora). \mocc saves about \wait{xx} percentage of time efficiency in model convergence time. In addition, we deep dive to show \mocc good results in terms of performance (throughput, latency, loss) fairness guarantees, friendliness towards legacy TCP , and robustness, in other words, reactivity to changing network conditions.
%
%\yq{8.Highlight}

%By no means do we expect that \mocc is the end of the story. Learn, remember and quickly apply policies under different applications is a hard job. However, \mocc represents a substantial overall advance, showing how a strong multi-objective learning-theoretic basis yields practical improvements.


==> sections/2background.tex <==
\section{Motivation}\label{sec:motivation}%\vspace{-1mm}
\vspace{-0.15in}

\subsection{Application Requirements}\label{subsec:appreq}
\vspace{-0.1in}

Internet applications have diverse performance requirements for the network,
typically characterized by metrics such as throughput, latency, jitter, and packet
loss rate~\cite{qos,ar,vr,vsnetwork,mmnetwork,kenyon1992audiovisual,silveira1999multimedia,szuprowicz1995multimedia}. Throughput is the main metric for many applications, in which minimum bandwidth is required to provide good user experience, e.g., HDTV requires 34Mbps to play high-definition video without rebuffering~\cite{qos}. On the other hand, real-time interactive
applications usually require low latency, e.g., autonomous driving requires low
latency ($<$15ms) to react to  immediate environment signals~\cite{qos1}. For
some real-time applications, temporal packet loss is also important, e.g.,
online video/audio conferencing can only tolerate $<$$0.1\%/1\%$ packet
loss rate~\cite{fluckiger1995understanding}. Emerging Internet applications such as
augmented/virtual reality may have tight requirements on several metrics. 
For example, augmented reality needs to operate under a
network environment of $>$100M bandwidth, $<$10ms delay, and $<$1\% packet
loss rate~\cite{qos1}.

These application demands pose requirements on Internet CC algorithms. Ideally,
the underlying CC algorithm should be: 1) {\em application-aware} to meet
individual application-specific demand, 2) {\em multi-objective} to support
multiple applications running  simultaneously, and 3) {\em quick-adaptive} to
accommodate new applications with new requirements. However, as we will show
subsequently ($\S$\ref{subsec:problem}), none of existing CC solutions can meet
these three goals simultaneously.

%Internet applications have diversified performance requirements for the network~\cite{qos,ar,vr,vsnetwork,mmnetwork,kenyon1992audiovisual,silveira1999multimedia,szuprowicz1995multimedia}, typically characterized by metrics such as throughput, latency (jitter), and packet loss rate, etc. Table~\ref{table:app} illustrates examples for some popular Internet applications and their performance requirements.

%For classic applications, throughput is often the main metric, and minimum bandwidth is required to be effective for some of them.
%, especially non-real-time multimedia players.
%For example, a HDTV requires a bandwidth of 34Mbps to play high-definition video without rebuffering~\cite{qos}. On the other hand, for real-time interactive applications, timely data delivery is more important for them to receive signals and make decisions. Thus, they have a stringent requirement on latency. For example, autonomous driving needs ultra low latency ($<$15ms) for vehicles to react to  immediate environment signals~\cite{qos1}. Furthermore, for some real-time applications, temporal packet loss also matters. Online video/audio conferencing is such an example, in which packets will be of no use if lost and retransmited after appropriate playback time. Thus, they only tolerate $<$$0.1\%/1\%$ temporal loss~\cite{fluckiger1995understanding}.
%For industrial control, any loss event of control signal is unacceptable~\cite{robot}.
%In addition, emerging Internet applications and servers such as augmented/virtual reality, IoT, and tactile Internet, etc., may have tight requirements on all the performance metrics. For example, augmented reality needs to operate under the network environment of $>$100M bandwidth, $<$10ms delay, and $<$1\% packet loss~\cite{qos1}.

%These application demands pose requirements on Internet CC algorithms. Ideally, the underlying CC algorithm should be: 1) {\em application-aware} to meet individual application-specific demand, 2) {\em multi-objective} to support multiple applications running  simultaneously, and 3) {\em quick-adaptive} to accommodate new applications with new requirements. However, as we will show subsequently ($\S$\ref{subsec:problem}), none of existing CC solutions can meet these three goals simultaneously.
%\vspace{-5mm}

%Due to the distinguishing characteristics, different applications have diversified performance requirements for the network. Figure \ref{fig:AppReq} presents the various quality of service metrics for many common and popular applications. For classic applications, bandwidth is the key metric. The assurance of minimum bandwidth is needed to fulfill basic function for many applications, especially non-real-time multimedia players. For example, a HDTV requires a bandwidth of 34MBit/s to play high-definition video without rebuffering. On the other hand, for interactive real-time applications, the timeliness of data delivery is very important for them to receive signals and make decisions instantaneously. Thus, they usually have a more stringent requirement on latency metric. For example, industrial control and autonomous driving require ultra low latency (<15ms) for robot arms and vehicles to timely react to the immediate environment signals. Furthermore, due to the property and usage of transferred data, the tolerance of data loss for different applications may be different. Though the correctness of data transfer can be guaranteed by using retransmission mechanism, for real-time applications, the loss may occur because a packet arrived too late to be useful. For example, for online video or audio conferencing, a packet will be of no use if arrives after its appropriate playback time, no matter caused by the delay in the network or being dropped and subsequently retransmitted. For industrial control and autonomous driving requiring both ultra low latency and preciseness, one loss event of control signal is unacceptable.

%Different applications have preferences for different metrics, and these preferences have different levels and need to be elaborately inspected with a fine-grained view. While lost data might result in a small glitch in the played-out audio/video, it may be cause serious and permanent impairment for a robot control program. Emerging applications such as virtual reality and Tactile Internet have tight requirements on all indexes. The challenge for the network is how to fit to different application requirements simultaneously in a fine-grained level.

\vspace{-0.18in}
\subsection{Problems of existing CC in supporting multiple application requirements}\label{subsec:problem}
\vspace{-0.12in}

We broadly classify existing Internet CC algorithms into two main categories: hand-crafted heuristics~\cite{newreno,cc,xcp,vegas,illinois,westwood,cubic,fast,compound,copa,bbr} and learning-based schemes~\cite{remy,allegro,vivace,aurora}. Below, we explain the problems of each category, with showcase examples. For brevity, we only use TCP CUBIC/Vegas~\cite{cubic,vegas} for the first category, and Aurora~\cite{aurora} for the second category here. All other algorithms share the similar trend as we validate in $\S$\ref{sec:eva}.

\parab{Hand-crafted CC:}The fundamental problem with hand-crafted CC is that most heuristic algorithms have no explicit application-aware utility function and hardwiredly map packet-level events to pre-defined reactions based on pre-assumptions of the network and experiences of human, thus hard to achieve optimal application-specific performance, not to mention supporting multiple applications.

Figure~\ref{fig:moti} illustrates the performance of different CC algorithms for throughput-sensitive application (a) and latency-sensitive application (b). In this experiment, the link bandwidth varies between 20-30Mbps, one-way delay is 50ms, and random packet loss ratio is 0.02\%. In general, we observe that TCP CUBIC is good (not the best) for throughput but bad for latency, whereas Vegas is good (not the best) for latency but bad for throughput. Such trend is expected, because: 1) these two schemes were designed with no explicit optimization goal in mind, but implicitly guide overall network behaviors with control rules, thus while they may obtain certain performance (e.g., CUBIC for throughput, Vegas for latency), they cannot ensure optimality; 2) they made assumptions about the network and applied pre-determined rules using experiences, thus suffering from performance degradation when actual network conditions deviate from pre-assumptions. For example, CUBIC assumes loss is caused by congestion and decreases the rate upon any occurrence of loss, leading to inferior throughput in the presence of non-congestion random loss as shown in Figure~\ref{fig:moti}a. \vspace{-1mm}

\begin{figure*}[ht]
\vspace{-10mm}
\centering
\subfigure[Single-objective CC (Aurora~\cite{aurora})] {
	\includegraphics[width=0.42\textwidth]{image/socc.pdf}
}
\subfigure[Multi-objective CC (MOCC)]{
	\includegraphics[width=0.53\textwidth]{image/mocc.pdf}
}
\vspace{-2mm}
\caption{From single-objective CC to multi-objective CC: Incorporating preference sub-network into MOCC with application requirements explicitly used in both state input and dynamic reward function enables \sys to learn (and memorize) the correlations between application requirements and the corresponding optimal rate control policies, thus realizing multi-objective, i.e., one single \sys model can support multiple applications.}
\label{fig:somo}
\vspace{-0.2in}
\end{figure*}

 %Figure~\ref{fig:moti}(a) plots the throughput of bandwidth-sensitive application. The network link\'s capcity bandwidth dynamic changes between 30-40 Mbps, one-way latency is 50 ms and random loss ratio is 1.5$\%$. We compare three congestion control schemes, one is TCP CUBIC, Linux\'s default; one is Vegas; and PCC-Aurora, RL-based congestion control. We observe that Vegas achieve the lowest throughput, TCP CUBIC although better than Vegas, still fails to effectively utilize the link\'s bandwidth due to the randomly packet loss. This is beacuse heuristic method is based on established experience. \eg CUBIC experience let it halve the sending rate upon any occurance of loss, which indiscriminate the application\'s high-bandwidth requirement. So hueristic method is not \emph{application-aware}, not to mention \emph{multi-objective}.

%In contrast, RL-based Aurora maintain high link utilization. This is because Aurora is \emph{application-aware}, it is specially designed for thorughput capturing. So it ignores the random loss and it works well for this bandwidth-sensitive application.

%We evaluate different CC schemes\'s throughput utilization under dynamic network bandwidth. We observe that handcraft CC CUBIC, which is famous for its bandwidth optimization. Handcraft CC Vegas, which is famous for its latency optimization, we observe from the Figure~\ref{fig:moti}(a)(b) that heurisitc method is not as good as the learning-based method, which is specially optimized for this object, like PCC-Aurora in the photo.

%\TODO{replaced with showcase results of heuristics} Based on heuristics derived from expert knowledge, the classic handcrafted CC algorithms construct hardwired mappings between predefined packet-level events and predefined control responses by hand. For example, TCP CUBIC assumes loss happens due to the network congestion and thus cut down the sending rate through a CUBIC equation. [One more example pls.] The assumptions made by experts in these algorithms usually focus on optimizing the performance in terms of a predefined criterion. However, there is a gap between the predefined criterion and the applications' objectives. The criterion is handcrafted based on assumptions of application demands, such as [example1][example2]. It may not respect the real requirement of applications. Furthermore,  the classical algorithms fix the criterion; changing it requires a lot of human efforts to explore the new hardwired mapping to optimize the new criterion. Thus, they cannot cater to different applications' objectives at the same time. Figure [] shows the performance of some traditional congestion control algorithms in terms of different metrics. [......description of the figure]

\parab{Learning-based CC:} State-of-the-art learning-based CC algorithms (e.g., Aurora~\cite{aurora}) can address the above problem of hand-crafted heuristics by explicitly expressing application-specific performance objective in reward function and maximizing it through machine learning from network environments, instead of human experiences. However, the key problem is that they can only optimize for a single objective at a time (see $\S$\ref{sec:MORL}). Supporting multiple applications requires multiple models. Furthermore, adapting to a new application entails re-training from scratch which takes time, making it neither multi-objective nor quick-adaptive.

From Figure~\ref{fig:moti}a\&b, we can see that Aurora performs the best in terms of both throughput and latency. However, this requires two different Aurora models (the same neural network structure but with different weights on edges) optimized for throughput and latency, respectively. Furthermore, as shown in Figure~\ref{fig:moti}c, re-training the model for a new application requirement takes long time, which is undesirable.

\parab{QUIC:} QUIC~\cite{quic} is a user-space transport protocol on top of UDP
to improve the transport performance of Internet applications and to enable
application-specific customizations. QUIC itself, however, is not tied to a
specific CC algorithm. It only provides the \emph{mechanism} to implement
application-specific CC algorithms, and an application still needs to specify
which CC it uses, which can be either hand-crafted or learning-based, to achieve
its performance objective. As such, our work is orthogonal to QUIC, and more
importantly, we show that we only need a single CC to satisfy all applications.

%\TODO{to polish, by Kai} Figure~\ref{fig:moti}(b) plots the latency of time-sensitive application. The network link\'s capacity bandwidth dynamic changes between 20-30 Mbps, one-way latency is 50 ms and random loss ratio is 0$\%$. We compare four congestion control schemes, TCP CUBIC, Vegas and two PCC-Aurora, one is optimized for throughput, another is optimized for latency. We observe that TCP CUBIC results in huge delay. Vegas, although better than TCP CUBIC, stills result in relatively high delay. Both heuristic method perform worse than PCC-Aurora. However, PCC-Aurora is originally optimized for throughput, which results in aggressive react and fierce latency jitter, high delay. So we specially trained PCC-Aurora to optimize for latency. As expected, PCC-Aurora optimized for latency is  better than PCC-Aurora optimized for throughput for time-sensitive application. This is because learning-based method is application-aware, and could be retrained for different kinds of objectives. But it takes time.

%We evaluate the time it takes \mocc to train for a specially-designed object in Figure~\ref{fig:moti}(c). We observe that it takes almost an hour to train the new model. This is not desirable in practical applications.


%\TODO{replaced with showcase results of existing learning CC} Inspired by the success of machine learning in various areas, recent proposals investigate learning-based approaches[][][]. Instead of constructing hardwired mappings as in classical handcrafted algorithms, learning-based CC algorithms use parametric models such as neural networks to represent the mapping.  They define the utility/reward function firstly and then apply machine learning techniques (e.g., gradient descent) to tune the model's parameters to maximize it. Thus, learning-based algorithms can directly optimize specific application-specific utility functions, granting them the capability of meeting different applications' demands. [Example: PCCRL] However, as the name says, learning-based CC algorithms require a learning/training process on the network environment to obtain an effective model optimizing on a specific objective. [Example: Remy, PCCRL] Thus, multiple applications running at the same time requires multiple models, and meeting every new coming appilcation demand involves a training process from scratch, which is both memory and time consuming. Also, the long training time before adapting to a new objective makes it impractical for meeting applications with different requirements simultaneously. PCC and PCC Vivace apply an online learning scheme to explore profitable actions and save the offline training process. However, the training cost is in fact amortized over the exploration steps, which leads to a sub-optimal adaptation rate to either dynamic network condition or new application requirement.

%\tianhan{Should we use an individual motivation experiment here, or refer to the quick adaptation experiment section?}
%We test how long it will take a reinforcement learning-based congestion control algorithm PCC-Aurora to adapt its policy to a new application requirement. As shown in the figure [], [...no matter we restart training from scratch or learn from a previously learned policy which is benefit for other application's preference. They are both time consuming. It takes PCC-Aurora 1 hour to converge when it choose to restart train the model. And it takes PCC-Aurora 20 mins to converge when it choose to transfer from the previous learned policy. Both of the methods fail in real internet due to the large amount of applications and the short response time that applications could endure. In contrast, a protocol designed within our MOCC framework could adjust its policy efficiently, this approximates the desired behavior. Our MOCC framework could apply the update policy within the application sustain time and appropriate for real internet applications....]

\vspace{-0.2in}
\subsection{Design Goals}\label{subsec:goal}
\vspace{-0.1in}

We seek {\em one single CC algorithm} satisfying all the following three goals simultaneously.
\begin{icompact}
%\vspace{-2mm}
\item \textbf{Application-aware}: The algorithm can automatically choose the optimal sending rates according to application-specific requirements without making any pre-assumptions of the network.
\item \textbf{Multi-objective}: The algorithm can support multiple heterogeneous applications running simultaneously, and provide the optimal policies for different applications, even with conflicting requirements.
\item \textbf{Quick-adaptive}: The algorithm can quickly adapt to new applications with unseen requirements, without compromising performance of old applications.
\end{icompact}
We are inspired by recent trend (notably, Aurora~\cite{aurora}) to adopt RL for CC, which can readily achieve application-awareness. However, the challenge is how to simultaneously support multiple applications and quickly accommodate new arrival ones. In the following, we establish a multi-objective RL framework for CC ($\S$\ref{sec:MORL}) to address this challenge.

%As the learning-based mechanism is necessary to guarantee the application-aware property, the key challenge to fulfill all three goals is to solve the contradiction between learning towards a single objective and meeting multiple objectives.

\iffalse
\begin{figure}
  \centering
  \includegraphics[width=8cm]{image/Figure4.png}
  \caption{A comparative picture of PCC-Aurora reward convergence picture}
  \vspace{-2em}
\end{figure}
\fi




==> sections/4.4Implementation.tex <==
%\vspace{-0.12in}
\subsection{Implementation}\label{subsec:implement}
%\vspace{-0.12in}

Our implementation of \mocc mainly consists of two components: 1) offline training, and 2) online deployment.

%three major parts: 1) offline training simulator; 2) \mocc online adaption library; 3) application integration layer. and more details will be covered in \S\ref{subsec:implement}.

\parab{Offline training:} Directly training \mocc in real environment is slow considering the actual time cost in real control loops of CC with complex network dynamics~\cite{chen2018auto,aurora,pensieve}. To enable efficient training, we train \sys in a networking simulator that faithfully mimics Internet links with various characteristics. Our simulator is based on OpenAI Gym~\cite{openai} and Aurora~\cite{aurora}, and further incorporates new design elements in $\S$\ref{subsec:architecture}--$\S$\ref{subsec:offline} that are essential to \sys, such as the encapsulation of application requirements as state input and dynamic reward functions.


\mocc policy network uses a fully-connected MLP(Multi-layer perceptron) with two hidden layers of 64 and 32 units, respectively, and \texttt{tanh} activation function to output the mean and standard deviations of the Gaussian distribution of action. The critic network uses the same neural network structure to estimate the scalar value function. We control the entropy factor $\beta$ to decay from 1 to 0.1 over 1000 iterations, and set clipping threshold $\epsilon=0.2$. 
For the learning rate, we adopt Adam~\cite{adam}, a famous adaptive learning rate optimization algorithm, swhich consistently outperforms standard SGD method. Important training parameter settings are listed in Table~\ref{tab:para}. We implement our model architecture with TensorFlow 1.14.0. For PPO implementation, we use an open-source implementation of several reinforcement learning baselines\footnote{https://github.com/hill-a/stable-baselines}.

To further accelerate \mocc's exploration towards optimal solutions for massive objectives, in addition to the two-phase training introduced in $\S$\ref{subsec:offline}, we also adopt parallel training. We implemented this architecture using Ray~\cite{ray} and RLlib~\cite{rllib} to build the multiple parallel environments. For compatibility, we leverage Ray API to declare the neural network during both training and testing.
\begin{table}[t]
%   \setlength{\abovecaptionskip}{0.1cm}
%   \setlength{\belowcaptionskip}{-0.3cm}  
  \begin{center}
   \begin{tabularx}{0.8\columnwidth}{c|c}
    \hline
    Parameter & Value\\
    \hline
    \hline
       Discount factor ($\gamma$) & 0.99 \\
       Learning rate ($\epsilon$) & 0.001 \\
       Action scale factor ($\alpha$) & 0.025 \\
       History length ($\eta$)& 10 \\    
       Landmark objectives \# ($\omega$) & 36 \\
    \hline
   \end{tabularx}
   % \vspace{-0.1in}
   \caption{Parameter settings}
    \label{tab:para}
    \vspace{-0.1in}
  \end{center}
 \end{table}




%\parab{Offline training} Directly training \mocc in realistic environment is not practical due to the complicated and uncontrolled network dynamics. To enable accurate and efficient training, we use offline training in a networking simulator. The simulator is based on OpenAI Gym~\cite{https://openai.com/}, which is a widely adopted toolkit to implement RL. The simulator is provided by Aurora, but we do several adjustments to the simulator to make it more fit to train \mocc model. 
%
%We provide application requirements to cooperate with our \mocc preference sub-network. The original sender in the simulator is an agent in the network with a rate, route and list of observations. Now, it gets one additional feature, \emph{application requirement}. This feature tells the agent how much the sender cares about each objective: throuhgput, latency and loss. The reward provided by the simulator is changed simultaneously with the applcation requirement. Also, the application requirements provided by our simulator comes in an order which is same with the neighbour-hood weight order.
%
%To easily explain how our enhanced simulator works. The gym simualtor use two link and a single Sender objects. At the begining, the links are initialized with bounded random values for bandwidth, latency que ue size and loss rate. The Sender initialized with an applciation requirement and a initial sending rate. Then the sender begins to take actions, the model begins to interact with simulated environments and experience with positive reward are reinforced.The detail value are discussed later in $\S$~\cite{sec:eva}. 
%
%To train our model, \mocc passes history length=10 past network measurements (including latency ratio,latency gradient and send ratio) aggregated with the 3-weight application requirements vectors in a hidden layer that uses 32 neurons to apply the tanh activation function to output the mean and variance (Figure 4). Then these two value are used as input into a network \yq{xudong structure} to generate the distribution of the actions. Then we could sample the action from the action distribution. The critic network uses the same NN structure, but its output a linear neuron to guide the loss update. During training, we use a discount factor $\lambda = 0.99$, which implies that current actions will be influenced by 100 future steps. The learning rates for the actor and critic are configured to be \wait{xx} and \wait{xx}, respectively. the entropy factor $\beta$ is controlled to decay from 1 to 0.1 over \wait{xx} iterations. Important parameter settings are listed in Table~\ref{tab:para}. 
%
%We keep all these hyperparameters fixed throughout our experiments. While some tunning is useful, we found that history length , the discount factor and learning rate is already discussed in aurora, so we borrow a good settinng validated by aurora. The undiscussed multi-objective related factor weights set size is discussed in $\S$~\cite{sec:eva}. 
%
%To accelerate \mocc's exploration towards optimal solutions for massive objectives, besides the two-phase training from theory perspective, we also adopt parallel training from engineering perspective. We implemented this architexture using Tensorflow Ray~\cite{ray} and RLlib~\cite{rllib} to build the multiple parallel environments. For compatibility,we leverage TF Ray API to declare the neural network during both training and testing.

%\TODO{Yiqing, what's this?} \wait{xx do we have this} Each environment is configured with different network conditions and application requirements and assigned one agent. We have one central agent to asynchronously aggregate the results from all other agents. By increasing the parallelism, we can further speedup the training progress.

%In our simulator, we first design and implement the neural networks of actor and critic networks. Both neural network has two hidden layer, with 32 and 16 neurons respectively and the activation function is $tanh$. We use Adam~\cite{adam} as the learning rate optimization algorithm. 
 
 
\parab{Online Deployment:} After the \mocc model was offline trained in the simulator, it needs to be online deployed with the real Internet applications. For better portability, we encapsulate all \mocc's functions into one library. Our library provides three main functions:
\begin{icompact}
	\item \texttt{Register($w$)}. Before using \mocc, we should register with it by providing the requirement/preference (weight vector $w$) of the application.
	\item \texttt{ReportStatus($s_t$)}. At each time interval, we should report the latest networking status ($s_t$) to \mocc.
	\item \texttt{GetSendingRate( )}. When sending packets, we use this function to obtain the sending rate calculated by \mocc.
\end{icompact}
With clean encapsulation, \mocc becomes an easy-to-use module and can be deployed with any networking datapaths.

In our implementation and evaluation, we integrate \mocc with UDT~\cite{udt} and CCP~\cite{ccp}. UDT is a user-space implementation and mostly used by video steaming applications. The \texttt{shim-helper} in UDT will interact with \mocc library and obtain the sending rate. CCP is a more general solution and enables congestion control outside datapath, such as Linux kernel networking stack. We integrate \mocc with CCP for more general-purpose applications. In $\S$\ref{subsec:realapp}, we use \sys to support three real Internet applications: video streaming, real-time communications, and bulk data transfer. We will introduce a bit more implementation details there.

%Once \mocc model was offline trained in the simulator, it could apply the congestion control policy to the real internet applcation and to evaluation.

%\textbf{\mocc Library}
%We encapsulate all \mocc's functions into one library for better portability. In our paper, we integrate \mocc to work with UDT~\cite{udt} and CCP~\cite{ccp}, and due to good abstraction of our library, \mocc can further be expended to work with other networking facility such as DPDK~\cite{} and others.\yq{what is DPDK?}
% 
%Our library provides three major functions:
%\begin{itemize}
%	\item \texttt{Register($W$)}. Before using \mocc, we should register our application with \mocc by providing the preference (in the weight vector $W$) of the application.
%	\item \texttt{ReportStatus($s_t$)}. At each timestep(TODO{please check} such as receiving an ACK), we should report the latest networking status ($s_t$) to \mocc.
%	\item \texttt{ReturnSendingRate()}. When we need to send packet, we can use this function to obtain the desired sending rate calculated by \mocc.
%\end{itemize}
%
%By clean encapsulation, \mocc becomes a practical and easy-to-use solution and can be deployed with any networking datapaths.
%
%\textbf{Application integration layer} 
%
%In our paper, we integrate \mocc with UDT and CCP. UDT is a use-space implementation and mostly used by video steaming applications~\cite{}. \texttt{shim-helper} in UDT will interact with \mocc's library and obtain the sending rate. 
%
%CCP is a more general solution and enables congestion control outside datapath, such as Linux kernel networking stack. We integrate \mocc with CCP for more general purpose applications, such as file transfer and so on.
%
%Please note, our application integration layer is a shim layer, which confirms it is very easy to plug \mocc with other networking datapaths.

%\yq{how to rewrite here ?}To train congestion control algorithm, \mocc designs the policy network with two hidden layers, each with 32, 16 neurons respectively. The default non-linearity is $\tanh$. The critic network uses the same NN structure with the actor. During training, we use a discount factor $\gamma= 0.99$, which implies that current actions will be influenced by 100 future steps. The optimizer for the actor and critic are configured to be Adam~\cite{adam} with learning rate 0.001. The weight of entropy loss is 0.01. The timesteps per update is 8192 and the optimizer's batchsize is 2048. For convenience, we use the well-structured deep reinforcement learning frameworks stable baselines and leverage PPO to implement the above framework. Other parameters are as the default configuration of PPO1. Additionally, the default size of weights set is 36. The table~\ref{tab:para} shows all parameters.

%To apply our \mocc algorithm for real congestion control task, we implement \mocc in both user and kernel space. 

%We implemented the data plane of \mocc in user space by adapting the UDP-based TCP skeleton in the UDT~\cite{udt} package. The control plane, named shim-helper, is implemented in Python for controlling the sending behavior of data plane. On the creation of each Monitor Interval, data plane will invoke the controller in control plane to get the corresponding sending rate.

%First \mocc was trained in randomized emulation environments. We elaborated Mahimahi~\cite{mahimahi}  to create the emulation links via specific bandwidth, latency and random loss rate. It sends real packets using a real Linux stack across virtual network interfaces using standard networking primitives. For easy training, we wrapped the data plane into a Gym-like Environment, which has unified interfaces for feasible training with some famous dedicated RL frameworks OpenAI~\cite{openai}. On each RESET, we create the network environment with UDT and Mahimahi. At each STEP, the rate controller (in Shim\_env) will determine the sending rate adjustment, named $\delta$, for data plane through the observation $s_{t-1}$ of last STEP and pass the rate changing to shim-helper by a TCP socket. Then the shim-helper will use $\delta$ to generate a new sending rate for further creation of monitor intervals. Once the MI ends, the statistical reports $s_t$ will be passed to shim-helper and further be sent to Shim-env to get next rate adjustment using the socket.

%In order to speed up the training process, we adapts Ray~\cite{ray} and RLlib~\cite{rllib} to increase the parallelism of network environments. 

%In test phase, we only need to configure a shim-helper with a pre-trained model to direct the sending processing in UDT framework.

%CCP (Congestion Control Plane)~\cite{ccp} is a new platform for writing and sharing datapath-agnostic congestion control algorithms. CCP provides the functionality for implementing complex congestion control algorithms in by placing them in a separate agent outside the datapath(\eg Linux Kernel TCP). The datapath can summarize the information about packets transmission process and pass it to user-defined congestion control algorithms, where the information will be mapped to a modification of congestion window or pacing rate. 

%In order to evaluate the performance in Linux Kernel~\cite{linux}, we leverage CCP~\cite{ccp} to make \mocc control the sending rate (pacing rate) of naive Linux Kernel TCP. We used the well-defined interfaces of CCP for getting the summary about sending behavior in datapath and giving back the control semantics that are generated by our pre-trained \mocc.



==> sections/6.1evaluation-setup.tex <==
%\subsection{Evaluation Setup}\label{subsec:setup}

\begin{figure*}
\vspace{-0.2in}
 \includegraphics[width=\textwidth] {image/label.pdf}
 \center
    \label{fig:label}
\end{figure*}
\begin{figure*}
  \vspace{-0.25in}
\centering
\subfigure[Varying bandwidth.]{\includegraphics[width=0.225\textwidth] {image/bw-utilization.pdf}\label{fig:multi11}}
\subfigure[Varying latency.] {\includegraphics[width=0.225\textwidth]{image/delay-utilization.pdf}\label{fig:multi12}}
\subfigure[Varying random loss.] {\includegraphics[width=0.225\textwidth] {image/loss-utilization.pdf}\label{fig:multi13}}
\subfigure[Varying buffer size.] {\includegraphics[width=0.225\textwidth] {image/buffer-utilization.pdf}\label{fig:multi14}}
  \vspace{-0.3in}
\quad
\subfigure[Varying bandwidth.]{\includegraphics[width=0.225\textwidth] {image/bw-latency.pdf}\label{fig:multi21}}
\subfigure[Varying latency.] {\includegraphics[width=0.225\textwidth]{image/delay-latency.pdf}\label{fig:multi22}}
\subfigure[Varying random loss.]{\includegraphics[width=0.225\textwidth] {image/loss-latency.pdf}\label{fig:multi23}}
\subfigure[Varying buffer size.]{\includegraphics[width=0.225\textwidth] {image/buffer-latency.pdf}\label{fig:multi24}}
\quad
  \vspace{-0.3in}
\caption{The multi-objective performance of \sys in terms of throughput (a-d) and latency (e-h), under varied network conditions. Note that the network conditions under evaluation are far beyond the environment where \sys was trained, demonstrating both its high performance and robustness when adopted in practicehhhhhhhhhhhhhhhhhhh.}\label{fig:multi1}
  \vspace{-0.3in}
\end{figure*}

%\iffalse
%\begin{figure*}
%  \centering
%  \vspace{-6pt}
%  \includegraphics[width=\textwidth]{image/loss-good.pdf}
%  \label{fig:lossgood}
%  \caption{packet loss ratio in different network condtions}
%\end{figure*}
%\fi

\parab{Settings:} Following $\S$\ref{sec:implement}, we use CCP to deploy our \mocc in both real Internet and Pantheon~\cite{pantheon} emulated environment. We train \mocc with varied bandwidth, latency, queue size and loss rate to cover a wide range of network conditions following the settings of prior works~\cite{aurora,pantheon}. The key parameters used in both training and evaluation are shown in Table~\ref{table:range}. In particular, when evaluating \mocc, we use a much wider parameter range beyond training to show the robustness of \sys.


\begin{table}[t]
\small
\vspace{-0.2in}
  \begin{tabular}{c|c|c|c|c}
    \hline 
     & Bandwidth & Latency & Queue size & Loss rate\\
    \hline 
    \hline
    Training & 1-5 Mbps & 10-50ms & 0-3000 pkts & 0-3\% \\
    \hline 
    Testing & 10-50 Mbps & 10-200ms & 500-5000 pkts & 0-10\% \\
    \hline 
  \end{tabular}
  %\vspace{-0.1in}
  \caption{Training/Testing parameters}
  \label{table:range}
  \vspace{-0.3in}
\end{table}

%To inspect the robustness of our congestion control algorithm to real-world the variety of network conditions, the testing suite have a range 10x larger than the training environment as showed in the table. 

\parab{Schemes compared:} We compare \mocc with various CC algorithms, including both handcrafted and learning-based:
\begin{enumerate}

\item Aurora~\cite{aurora}, RL based CC algorithm, single-objective (thus Aurora-throughput and Aurora-latency use two separate models).
\item Orca~\cite{orca}, RL based CC algorithm, which combine the classic CC with advanced RL techniques to achieve low overhead and better performance.
\item PCC Allegro~\cite{allegro}, learning-based, performs \emph{micro experiments} to continuously explore and learn the target sending rate.
\item PCC Vivace~\cite{vivace}, learning-based, extends upon Allegro to achieve better performance.
\item BBR~\cite{bbr}, model-based heuristic, builds an explicit model based on available bandwidth and RTT, and uses the model to control congestion window.
\item Copa~\cite{copa}, delay-based heuristic, computes the target sending rate by estimating minimum delay.
\item TCP CUBIC~\cite{cubic}, loss-based heuristic, when packets are dropped, CUBIC modulates its congestion window based on a CUBIC function.
\item TCP Vegas~\cite{vegas}, delay-based heuristic, uses RTT as congestion signal and controls congestion window to maintain desired RTT.
%\item Comound,\TODO{not compared but introduced}, loss and delay-based handcrafted heuristic, Compound reacts to delay signals and packet loss events and adopts a scalable increasing rule on cwnd in response to changes inn the RTTs.
%\item Remy, \TODO{not compared but introduced}, learning-based, RemyCC formalizes the multiuser CC problem as the POMDP and learns the optimum offline policy under a wide range of network environments.
%\item PCC Allegro and Vivace~\cite{allegro,vivace}, learning-based. PCC continuously performs \emph{micro-experiments} to learn the target sending rate.
% adaptively adjusts its sending rate based on continuously carried out "micro-experiments", and online choose the action which could maximize the PCC utility funcntion.
%Aurora proposed to use RL to design a TCP CC scheme, adjusting the sending rate according to the policy which could optimize the reward function. Here we trained two version of Aurora. We adjusted the reward function to make one model much prefer to capture throughput, another model much prefer to avoid increasing delay.
\end{enumerate}




%\parab{Metrics:} In our evaluation, applications are mainly classified as throughput-sensitive and delay-sensitive. For the former one, we measure the link bandwidth utilization achieved by different protocols; For the latter one, we measure the end-to-end latency delivered by them. We also evalute the satisfaction of an arbitrary application's requirment by measuring the cumulative reward gain in terms of its application objective as defined in \S\ref{subsec:architecture}.

%\parab{Metrics:} We mainly evaluate \mocc with both throughput-sensitive and delay-sensitive applications, and we measure the link bandwidth utilization and end-to-end latency respectively. Furthermore, we also evaluate the ability of satisfaction of applications' requirement by measuring its gained cumulative reward (defined in \S\ref{subsec:architecture}). We also assess the ability of how fast \mocc could adapt to new applications without compromising the old ones.







==> sections/8related.tex <==
\vspace{-0.15in}
\section{Related Work}\label{sec:related}%\vspace{-1mm}
%\vspace{-0.2in}
More than three decades of research on congestion control, have provided us with a plethora of  Internet congestion control schemes, e.g.,~\cite{newreno,cc,xcp,vegas,illinois, westwood,cubic,fast,compound, bbr, copa,remy,adaptivecc, allegro, learningcc,qtcp, vivace, custard,mlcc,tcpdrinc,aurora,orca,tcprl,rtcms,mvfst}.  Those learning-based algorithms proposed recently are related to our \sys. For space limitation, we do not introduce these efforts one by one. However, the key difference is that \sys is perhaps the first work that introduces a principled RL-based congestion control approach that achieves multi-objective and quick-adaptation, a challenging goal never realized in prior work. 



